Local-Global Methods for Generalised Solar Irradiance Forecasting

As the use of solar power increases, having accurate and timely forecasts will be essential for smooth grid operators. There are many proposed methods for forecasting solar irradiance / solar power production. However, many of these methods formulate the problem as a time-series, relying on near real-time access to observations at the location of interest to generate forecasts. This requires both access to a real-time stream of data and enough historical observations for these methods to be deployed. In this paper, we propose the use of Global methods to train our models in a generalised way, enabling them to generate forecasts for unseen locations. We apply this approach to both classical ML and state of the art methods. Using data from 20 locations distributed throughout the UK and widely available weather data, we show that it is possible to build systems that do not require access to this data. We utilise and compare both satellite and ground observations (e.g. temperature, pressure) of weather data. Leveraging weather observations and measurements from other locations we show it is possible to create models capable of accurately forecasting solar irradiance at new locations. This could facilitate use planning and optimisation for both newly deployed solar farms and domestic installations from the moment they come online. Additionally, we show that training a single global model for multiple locations can produce a more robust model with more consistent and accurate results across locations.

==> tables/local_global_rmse_overview.tex <==
\begin{tblr}{Q[r] |Q[c, 1cm] Q[c, 1cm]|[dashed] Q[c, 1cm] Q[c, 1cm]}
\toprule


     & \SetCell[c=2]{c} Global  & &  \SetCell[c=2]{c} Local \\

      & \ac{nRMSE}    & std   & \ac{nRMSE}   & std         \\ 
\hline
CNN	 & \textbf{\emph{0.213}}	& 0.038 &	0.241 &	0.042 \\ 
\hline[dashed]
DNN	 & \em{0.333}	& 0.067 &	0.397 &	0.074 \\
LSTM & 	\em{0.324}	& 0.069 &	0.375 &	0.090 \\ 
\hline[dashed]
Tree & 	0.343	& 0.057 &	\em{0.340} &	0.056 \\
\end{tblr}


==> tables/local_global_skill_overview.tex <==

\begin{tblr}{Q[r] |Q[c, 1cm] Q[c, 1cm]|[dashed] Q[c, 1cm] Q[c, 1cm]}
      & \SetCell[c=2]{c} Global  & &  \SetCell[c=2]{c} Local \\

      & \ac{nRMSE}    & std   & \ac{nRMSE}   & std         \\ 
\hline

CNN	 & \textbf{\em{0.837}} & 0.043 & 0.788 & 0.048 \\
\hline[dashed]
DNN	 & \em{0.741} & 0.055 & 0.706 & 0.055 \\
LSTM & \em{0.750} & 0.059 & 0.731 & 0.047 \\
\hline[dashed]
Tree & 0.547 & 0.159 & \em{0.540} & 0.179 \\

\end{tblr}

